Dual Strategies for Test-Time Adaptation

Conventional test-time adaptation (TTA) approaches typically adapt the model using only a small fraction of test samples, often those with low-entropy predictions, thereby failing to fully leverage the available information in the test distribution. This paper introduces DualTTA, a novel framework that improves performance under distribution shifts by utilizing a larger and more diverse set of test samples. DualTTA identifies two distinct groups: one where the model's predictions are likely consistent with the underlying semantics, and another where predictions are likely incorrect. For the first group, it minimizes prediction entropy to reinforce reliable decisions; for the second, it maximizes entropy to suppress overconfident errors and unlearn spurious behavior. These groups are adaptively selected using a new reliability criterion that measures prediction stability under both semantic-preserving and semantic-altering transformations, addressing the limitations of purely entropy-based selection. We further provide theoretical analysis and empirical justification showing that our approach enables a tighter separation between reliable and unreliable samples, in the context of their suitability for adaptation, leading to provably more effective model updates.

==> sec/X_checklist.tex <==
\maketitlechecklist

% This paper:
% \begin{itemize}
%     \item Includes a conceptual outline and/or pseudocode description of AI methods introduced. (yes/partial/no/NA)\\
%     \textbf{\textit{Answer:}}\textcolor{blue}{[YES]}.
%     \item Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results. (yes/no)\\
%     \textbf{\textit{Answer:}}\textcolor{blue}{[YES]}.
%     \item Provides well marked pedagogical references for less-familiare readers to gain background necessary to replicate the paper. (yes/no)\\
%     \textbf{\textit{Answer:}}\textcolor{blue}{[YES]}.
% \end{itemize}
% Does this paper make theoretical contributions? (yes/no)
% \textbf{\textit{Answer:}}\textcolor{red}{[NO]}.

% If yes, please complete the list below.
% \begin{itemize}
%     \item All assumptions and restrictions are stated clearly and formally. (yes/partial/no)
%     \item All novel claims are stated formally (e.g., in theorem statements). (yes/partial/no)
%     \item Proofs of all novel claims are included. (yes/partial/no)
%     \item Proof sketches or intuitions are given for complex and/or novel results. (yes/partial/no)
%     \item Appropriate citations to theoretical tools used are given. (yes/partial/no)
%     \item All theoretical claims are demonstrated empirically to hold. (yes/partial/no/NA)
%     \item All experimental code used to eliminate or disprove claims is included. (yes/no/NA)
% \end{itemize}
% Does this paper rely on one or more datasets? (yes/no)\\
% \textbf{\textit{Answer:}}\textcolor{blue}{[YES]}.

% If yes, please complete the list below.
% \begin{itemize}
%     \item A motivation is given for why the experiments are conducted on the selected datasets. (yes/partial/no/NA)\\
%     \textbf{\textit{Answer:}}\textcolor{blue}{[YES]}.
%     \item A motivation is given for why the experiments are conducted on the selected datasets. (yes/partial/no/NA)
%     \item All novel datasets introduced in this paper are included in a data appendix. (yes/partial/no/NA)
%     \item All novel datasets introduced in this paper will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no/NA)
%     \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are accompanied by appropriate citations. (yes/no/NA)
%     \item All datasets drawn from the existing literature (potentially including authors’ own previously published work) are publicly available. (yes/partial/no/NA)
%     \item All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing. (yes/partial/no/NA)
% \end{itemize}
% Does this paper include computational experiments? (yes/no)

% If yes, please complete the list below.
% \begin{itemize}
%     \item This paper states the number and range of values tried per (hyper-) parameter during development of the paper, along with the criterion used for selecting the final parameter setting. (yes/partial/no/NA)
%     \item Any code required for pre-processing data is included in the appendix. (yes/partial/no).
%     \item All source code required for conducting and analyzing the experiments is included in a code appendix. (yes/partial/no)
%     All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes. (yes/partial/no)
%     \item All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from (yes/partial/no)
%     \item If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results. (yes/partial/no/NA)
%     \item This paper specifies the computing infrastructure used for running experiments (hardware and software), including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks. (yes/partial/no)
%     \item This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics. (yes/partial/no)
%     \item This paper states the number of algorithm runs used to compute each reported result. (yes/no)
%     \item Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information. (yes/no)
%     \item The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank). (yes/partial/no)
%     \item This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments. (yes/partial/no/NA)
% \end{itemize}
\begin{enumerate}
  \item \textbf{Includes a conceptual outline and/or pseudocode description of AI methods introduced.}\\  
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.\\
    \textbf{\textit{Justification:}}
    We give a full conceptual outline of DualTTA (Sec. 3) and detail the algorithmic pipeline in Figure ~\ref{fig:overview}.  
  \item \textbf{Clearly delineates statements that are opinions, hypothesis, and speculation from objective facts and results.}\\
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.
  \item \textbf{Provides well marked pedagogical references for less-familiar readers to gain background necessary to replicate the paper.}\\
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.
  \item \textbf{Does this paper make theoretical contributions?}\\ 
    \textbf{\textit{Answer:}} \textcolor{red}{[NO]}. \\
    \textbf{\textit{Justification:}} Our contributions are methodological and empirical; we do not state formal theorems or proofs.
\end{enumerate}

\noindent\textbf{If yes, please complete the list below.}  (Skipped since no theoretical claims.)

\bigskip
\noindent\textbf{Dataset use}
\begin{enumerate}\setcounter{enumi}{4}
  \item \textbf{Does this paper rely on one or more datasets?}  \\
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.\\
    \textbf{\textit{Justification:}} We evaluate on ColoredMNIST, Waterbirds, PACS, Office‑Home, and ImageNet‑C.
  
  \item \textbf{A motivation is given for why the experiments are conducted on the selected datasets.}\\  
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.\\
    \textbf{\textit{Justification:}} Sec.~4.1 explains the choice of each benchmark to test spurious correlation, domain‑shift, and corruption robustness.
  
  \item \textbf{All novel datasets introduced in this paper are included in a data appendix.} \\ 
    \textbf{\textit{Answer:}} \textcolor{pink}{[NA]}.\\
    \textbf{\textit{Justification:}} We do not introduce any new datasets.
  
  \item \textbf{All novel datasets introduced in this paper will be made publicly available upon publication}\\  
    \textbf{\textit{Answer:}} \textcolor{pink}{[NA]}.\\
    \textbf{\textit{Justification:}} We do not introduce any new datasets.
  \item \textbf{All datasets drawn from the existing literature are accompanied by appropriate citations.}\\  
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.
  \item \textbf{All datasets drawn from the existing literature are publicly available.}  \\
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.\\
    \textbf{\textit{Justification:}} All benchmarks used (ColoredMNIST, Waterbirds, PACS, Office‑Home, ImageNet‑C) are open‑access.
  
  \item \textbf{All datasets that are not publicly available are described in detail, with explanation why publicly available alternatives are not scientifically satisficing.}  \\
    \textbf{\textit{Answer:}} \textcolor{pink}{[NA]}.
\end{enumerate}

\bigskip
\noindent\textbf{Computational experiments}
\begin{enumerate}\setcounter{enumi}{12}
  \item \textbf{Does this paper include computational experiments?}  \\
  \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.
  \item \textbf{This paper states the number and range of values tried per (hyper‑)parameter during development of the paper, along with the criterion used for selecting the final parameter setting.}  \\
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES but not done!]}.
  
  \item \textbf{Any code required for pre‑processing data is included in the appendix.} \\
    \textbf{\textit{Answer:}} \textcolor{red}{[NO]}. \\
    \textbf{\textit{Justification:}} Data preprocessing follows standard scripts (e.g. torchvision transforms).
  
  \item \textbf{All source code required for conducting and analyzing the experiments is included in a code appendix.} \\ 
    \textbf{\textit{Answer:}} \textcolor{red}{[NO]}. \\
    \textbf{\textit{Justification:}} Code will be released publicly after publication.
  
  \item \textbf{All source code required for conducting and analyzing the experiments will be made publicly available upon publication of the paper with a license that allows free usage for research purposes.} \\ 
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.\\
    \textbf{\textit{Justification:}} We commit to open‑sourcing our implementation under a permissive license.
  
  \item \textbf{All source code implementing new methods have comments detailing the implementation, with references to the paper where each step comes from}  \\
  \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.
  \item \textbf{If an algorithm depends on randomness, then the method used for setting seeds is described in a way sufficient to allow replication of results.}  \\
  \textbf{\textit{Answer:}} \textcolor{blue}{[YES but not done!]}.
  \item \textbf{This paper specifies the computing infrastructure used for running experiments , including GPU/CPU models; amount of memory; operating system; names and versions of relevant software libraries and frameworks.}  \\
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES but not done!]}.
  
  \item \textbf{This paper formally describes evaluation metrics used and explains the motivation for choosing these metrics.}  \\
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.\\
    \textbf{\textit{Justification:}} We define Avg Acc and Worst Acc over group splits (Sec.~4.1) and justify their use for assessing robustness.
  
  \item \textbf{This paper states the number of algorithm runs used to compute each reported result.}  \\
    \textbf{\textit{Answer:}} \textcolor{red}{[NO]}.
  
  \item \textbf{Analysis of experiments goes beyond single-dimensional summaries of performance (e.g., average; median) to include measures of variation, confidence, or other distributional information.}  \\
    \textbf{\textit{Answer:}} \textcolor{red}{[NO]}.
  
  \item \textbf{The significance of any improvement or decrease in performance is judged using appropriate statistical tests (e.g., Wilcoxon signed-rank).}  \\
  \textbf{\textit{Answer:}} \textcolor{red}{[NO]}.
  
  \item \textbf{This paper lists all final (hyper-)parameters used for each model/algorithm in the paper’s experiments.} \\ 
    \textbf{\textit{Answer:}} \textcolor{blue}{[YES]}.\\
    \textbf{\textit{Justification:}} Sec.~4.2 (and App.~C) lists learning rates, thresholds ($\tau_{Ent},\tau_{ca},\tau_{sa}$), normalization factors, and layer positions.
\end{enumerate}


